Microstructural Smoothed Particle Hydrodynamics Model and Simulations of Discontinuous Shear-Thickening Fluids

Despite the recent interest in the discontinuous shear-thickening (DST) behaviour, few computational works tackle the rich hydrodynamics of these fluids. In this work, we present the first implementation of a microstructural DST model in Smoothed Particle Hydrodynamic (SPH) simulation. The scalar model was implemented in an SPH scheme and tested in two flow geometries. Three distinct ratios of local to non-local microstructural effects were probed: weak, moderate, and strong non-locality. Strong and moderate cases yielded excellent agreement with flow curves constructed via the Wyart--Cates (WC) model, with the moderate case exhibiting banding patterns. Weak non-locality produced stress-splitting instability, resulting in discontinuous stress fields and poor agreement with the WC model. The mechanism of the stress-splitting has been explored and contextualised by the interaction of local microstructure evolution and the stress-control scheme. Velocity profiles obtained in body force-driven channel flow were found to be in excellent agreement with the analytical solution, yielding an upward inflection corresponding to the typical S-curve. Simulations carried out at increasing driving forces exhibited a decrease in flow. We showed that even the simple scalar model can capture some of the key properties of DST materials, laying the foundation for further SPH study of instabilities and pattern formation.

==> bib_backup.tex <==
@article{Ellero2007,
title = {Incompressible smoothed particle hydrodynamics},
journal = {Journal of Computational Physics},
volume = {226},
number = {2},
pages = {1731-1752},
year = {2007},
issn = {0021-9991},
doi = {https://doi.org/10.1016/j.jcp.2007.06.019},
url = {https://www.sciencedirect.com/science/article/pii/S0021999107002598},
author = {Marco Ellero and Mar Serrano and Pep Español},
keywords = {Incompressible flows, Smoothed particle hydrodynamics},
abstract = {We present a smoothed particle hydrodynamic model for incompressible fluids. As opposed to solving a pressure Poisson equation in order to get a divergence-free velocity field, here incompressibility is achieved by requiring as a kinematic constraint that the volume of the fluid particles is constant. We use Lagrangian multipliers to enforce this restriction. These Lagrange multipliers play the role of non-thermodynamic pressures whose actual values are fixed through the kinematic restriction. We use the SHAKE methodology familiar in constrained molecular dynamics as an efficient method for finding the non-thermodynamic pressure satisfying the constraints. The model is tested for several flow configurations.}
}

@article{JFM2019, title={Shear thickening of a non-colloidal suspension with a viscoelastic matrix}, volume={880}, DOI={10.1017/jfm.2019.753}, journal={Journal of Fluid Mechanics}, publisher={Cambridge University Press}, author={Vázquez-Quesada, Adolfo and Español, Pep and Tanner, Roger I. and Ellero, Marco}, year={2019}, pages={1070–1094}}

@article{Muzio,
  title = {Transition to Turbulence and Mixing in a Viscoelastic Fluid Flowing Inside a Channel with a Periodic Array of Cylindrical Obstacles},
  author = {Grilli, Muzio and V\'azquez-Quesada, Adolfo and Ellero, Marco},
  journal = {Phys. Rev. Lett.},
  volume = {110},
  issue = {17},
  pages = {174501},
  numpages = {5},
  year = {2013},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.110.174501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.174501}
}


@article{PAIVA2009306,
title = {Particle-based viscoplastic fluid/solid simulation},
journal = {Computer-Aided Design},
volume = {41},
number = {4},
pages = {306-314},
year = {2009},
note = {Point-based Computational Techniques},
issn = {0010-4485},
doi = {https://doi.org/10.1016/j.cad.2008.10.004},
url = {https://www.sciencedirect.com/science/article/pii/S0010448508001887},
author = {Afonso Paiva and Fabiano Petronetto and Thomas Lewiner and Geovan Tavares},
keywords = {Viscoplastic fluid, Solid deformation, Smoothed particle hydrodynamics, Radial basis function, Non-Newtonian fluid, Physically-based animation},
abstract = {Simulations of viscoplastic materials are traditionally governed by continuum mechanics. The viscous behavior is typically modeled as an internal force, defined by diverse quantities. This work introduces a fluid model to simulate the viscoplastic effect of solid materials, such as plastic, wax, clay and polymer. Our method consists in modeling a solid object through a non-Newtonian fluid with high viscosity. This fluid simulation uses the Smoothed Particle Hydrodynamics method and the viscosity is formulated by using the General Newtonian Fluid model. This model concentrates the viscoplasticity in a single parameter. Our results show clear effects of creep, melting, hardening and flowing.}
}

@Article{Zhu2018,
author={Zhu, Chongqiang
and Huang, Yu
and Zhan, Liang-tong},
title={SPH-based simulation of flow process of a landslide at Hongao landfill in China},
journal={Natural Hazards},
year={2018},
month={Sep},
day={01},
volume={93},
number={3},
pages={1113-1126},
abstract={Landfills are the most popular means of disposing of construction solid waste owing to the low-cost, large treatment volume and strong adaptability. However, landfill collapses and landslides are common, posing a risk to lives and property. A catastrophic landslide, not triggered by heavy rainfall or earthquakes, occurred on December 20, 2015, at Hongao landfill in Guangming New district of Shenzhen, China. The collapsed waste soil flowed 1100 m down a slope with an elevation difference of 100 m. This catastrophic landslide is typical of long-runout disasters with high mobility, which result in great loss to life and property. In this paper, we focused on reproducing the flow processes and simulating the arriving area of the landslide at Hongao landfill using a full three-dimensional (3D) smoothed particle hydrodynamics (SPH) method. A series of undrained ring shear tests were conducted to determine the viscosity coefficient for the numerical simulation. The calculated geometry of the landslide using the full 3D SPH method agreed well with the field data. Hence, the combination of ring shear tests and SPH method can be widely used to predict the dynamic behavior of potential landslides in landfills, to reduce or prevent similar disasters.},
issn={1573-0840},
doi={10.1007/s11069-018-3342-8},
url={https://doi.org/10.1007/s11069-018-3342-8}
}



@article{ZHU2010362,
title = {A numerical study of the flow of Bingham-like fluids in two-dimensional vane and cylinder rheometers using a smoothed particle hydrodynamics (SPH) based method},
journal = {Journal of Non-Newtonian Fluid Mechanics},
volume = {165},
number = {7},
pages = {362-375},
year = {2010},
issn = {0377-0257},
doi = {https://doi.org/10.1016/j.jnnfm.2010.01.012},
url = {https://www.sciencedirect.com/science/article/pii/S0377025710000145},
author = {Huaning Zhu and Nicos S. Martys and Chiara Ferraris and Daniel De Kee},
keywords = {Vane rheometer, Smoothed particle hydrodynamics (SPH), Bingham fluid, Non-Newtonian fluid, Papanastasiou model},
abstract = {In this paper, a Lagrangian formulation of the Navier–Stokes equations, based on the smoothed particle hydrodynamics (SPH) approach, was applied to determine how well rheological parameters such as plastic viscosity can be determined from vane rheometer measurements. First, to validate this approach, a Bingham/Papanastasiou constitutive model was implemented into the SPH model and tests comparing simulation results to well established theoretical predictions were conducted. Numerical simulations for the flow of fluids in vane and coaxial cylinder rheometers were then performed. A comparison to experimental data was also made to verify the application of the SPH method in realistic flow geometries. Finally, results are presented from a parametric study of the flow of Bingham fluids with different yield stresses under various applied angular velocities of the outer cylindrical wall in the vane and coaxial cylinder rheometers. The stress, strain rate and velocity profiles, especially in the vicinity of the vane blades, were computed. By comparing the calculated stress and flow fields between the two rheometers, the validity of the assumption that the vane could be approximated as a cylinder for measuring the rheological properties of Bingham fluids at different shear rates was tested.}
}

@article{Khanpour,
title = {Mesh-free SPH modeling of sediment scouring and flushing},
journal = {Computers \& Fluids},
volume = {129},
pages = {67-78},
year = {2016},
issn = {0045-7930},
doi = {https://doi.org/10.1016/j.compfluid.2016.02.005},
url = {https://www.sciencedirect.com/science/article/pii/S0045793016300238},
author = {M. Khanpour and A.R. Zarrati and M. Kolahdoozan and A. Shakibaeinia and S.M. Amirshahi},
keywords = {Smoothed Particle hydrodynamics (SPH), Continuum-based sediment transport, Sediment scouring, Sediment flushing},
abstract = {A two-phase mesh-free Lagrangian model, based on the Smoothed Particle Hydrodynamics (SPH) method, is developed and evaluated for the continuum-based study of sediment-water system (a dense submerged granular flow system). The case studies are (a) sediment scouring downstream of a wall-jet, and (b) reservoir sediment flushing, both of great interest of engineers and researchers. The mesh-free Lagrangian nature of the SPH method makes the model capable of dealing with the large interfacial deformations involved in these complex water-sediment flow systems. Water and sediment materials are both treated as continuum and the governing equation of their motion are solved on a Lagrangian frame using SPH formulation. A pressure-dependent viscoplastic rheological model is used to describe the behavior of the sediment phase. A combination of Mohr–Coulomb and Shields yielding criteria (in place of commonly used Mohr–Coulomb yield criteria) is employed to determine the critical stress above which the sediment material behaves as a viscous fluid. Effect of this combination on the model results is investigated. To validate the developed numerical model, this study also provides some original experimental measurements for the test cases of this study. The results show the good compatibility of the numerical and experimental water and bed profiles. The sediment feature such as scouring and deposition areas (for wall-jet scouring case) and the sediment failure slope (for the flushing test case) are reproduced by the developed SPH model, with a good degree of accuracy. The numerical results as well as experimental measurements of this study not only provide an insight into better understanding of the complicated mechanism of sediment transport induced by rapid flow discharge, but also provide a reliable numerical tool and benchmark for simulation of such problems.}
}

@article{Fourtaka,
title = {Modelling multi-phase liquid-sediment scour and resuspension induced by rapid flows using Smoothed Particle Hydrodynamics (SPH) accelerated with a Graphics Processing Unit (GPU)},
journal = {Advances in Water Resources},
volume = {92},
pages = {186-199},
year = {2016},
issn = {0309-1708},
doi = {https://doi.org/10.1016/j.advwatres.2016.04.009},
url = {https://www.sciencedirect.com/science/article/pii/S0309170816300926},
author = {G. Fourtakas and B.D. Rogers},
keywords = {SPH, Multi-phase, Scouring, Sediment transport, Suspension, GPU},
abstract = {A two-phase numerical model using Smoothed Particle Hydrodynamics (SPH) is applied to two-phase liquid-sediments flows. The absence of a mesh in SPH is ideal for interfacial and highly non-linear flows with changing fragmentation of the interface, mixing and resuspension. The rheology of sediment induced under rapid flows undergoes several states which are only partially described by previous research in SPH. This paper attempts to bridge the gap between the geotechnics, non-Newtonian and Newtonian flows by proposing a model that combines the yielding, shear and suspension layer which are needed to predict accurately the global erosion phenomena, from a hydrodynamics prospective. The numerical SPH scheme is based on the explicit treatment of both phases using Newtonian and the non-Newtonian Bingham-type Herschel-Bulkley-Papanastasiou constitutive model. This is supplemented by the Drucker-Prager yield criterion to predict the onset of yielding of the sediment surface and a concentration suspension model. The multi-phase model has been compared with experimental and 2-D reference numerical models for scour following a dry-bed dam break yielding satisfactory results and improvements over well-known SPH multi-phase models. With 3-D simulations requiring a large number of particles, the code is accelerated with a graphics processing unit (GPU) in the open-source DualSPHysics code. The implementation and optimisation of the code achieved a speed up of x58 over an optimised single thread serial code. A 3-D dam break over a non-cohesive erodible bed simulation with over 4 million particles yields close agreement with experimental scour and water surface profiles.}
}

@Article{Jop2006,
author={Jop, Pierre
and Forterre, Yo{\"e}l
and Pouliquen, Olivier},
title={A constitutive law for dense granular flows},
journal={Nature},
year={2006},
month={Jun},
day={01},
volume={441},
number={7094},
pages={727-730},
abstract={Equations describing how granular materials move under shear are still a matter of debate. Jop et al. now propose a new model for dense granular flows in three dimensions, inspired by the behaviour of visco-plastic fluids such as toothpaste. The results could serve as a basic tool for modelling complex flows in geophysical or industrial applications.},
issn={1476-4687},
doi={10.1038/nature04801},
url={https://doi.org/10.1038/nature04801}
}



@article{Pouliquen_2006,
doi = {10.1088/1742-5468/2006/07/P07020},
url = {https://dx.doi.org/10.1088/1742-5468/2006/07/P07020},
year = {2006},
month = {jul},
publisher = {},
volume = {2006},
number = {07},
pages = {P07020},
author = {O Pouliquen and C Cassar and P Jop and Y Forterre and M Nicolas},
title = {Flow of dense granular material: towards simple constitutive laws},
journal = {Journal of Statistical Mechanics: Theory and Experiment},
abstract = {Recent experiments and numerical simulations of dry granular flows suggest that a simple rheological description in terms of a friction coefficient varying both with shear rate and pressure through a dimensionless inertial number may be sufficient to capture the major properties of granular flows. In this paper we first present the empirical constitutive laws and their interpretation using dimensional analysis, before analysing the prediction for different flow configurations. The successes and limits of the approach are discussed based on comparison with recent studies.}
}


@article{MinattiParis,
title = {A SPH model for the simulation of free surface granular flows in a dense regime},
journal = {Applied Mathematical Modelling},
volume = {39},
number = {1},
pages = {363-382},
year = {2015},
issn = {0307-904X},
doi = {https://doi.org/10.1016/j.apm.2014.05.034},
url = {https://www.sciencedirect.com/science/article/pii/S0307904X14002960},
author = {Lorenzo Minatti and Enio Paris},
keywords = {Smoothed Particles Hydrodynamics, Granular flows, Viscosity regularisation},
abstract = {Smoothed Particle Hydrodynamics (SPH) is a particle-based Lagrangian numerical method, particularly suitable for modeling free surface flows of fluids with different constitutive equations. In this work, a SPH model is developed to solve flow problems of granular matter flowing in a dense regime, featuring a constitutive equation proposed by Pouliquen et al. (2006) [17] and Jop et al. (2006) [18]. The problem of resolving the flow close to static conditions has been solved by introducing a weak compressibility for the grains: this leads to a third order algebraic equations to be solved for computing granular material density. A new viscosity regularisation method, suitable for any visco-plastic fluid with varying yield stress has been developed, in order to reproduce stopping flow and static conditions. Validation of the model has been performed by solving the simple uniform granular flow problem, for which the solution is known analytically and by reproducing a set of experimental data on granular columns collapses by Lube et al. (2004) [19].}
}

@article{BonetRodriguez-Paz,
author = {Rodriguez-Paz, M. X. and Bonet, J.},
title = {A corrected smooth particle hydrodynamics method for the simulation of debris flows},
journal = {Numerical Methods for Partial Differential Equations},
volume = {20},
number = {1},
pages = {140-163},
keywords = {SPH, debris flows, mesh-free method, avalanches},
doi = {https://doi.org/10.1002/num.10083},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/num.10083},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/num.10083},
abstract = {Abstract This article presents the development and application of a corrected smooth particle hydrodynamics (CSPH) code to the simulation of debris flow and avalanches. The advantages of a mesh-free method over other traditional numerical methods such as the finite element method are discussed. A new frictional approach for the boundary conditions and modified constitutive equations are introduced in the SPH method. The resulting technique is then applied for the simulation of debris flows, comparing the results with those obtained from experiments reported by other researchers. © 2003 Wiley Periodicals, Inc. Numer Methods Partial Differential Eq 20: 140–163, 2004.},
year = {2004}
}



@misc{moreno2023morphological,
      title={Morphological transitions of block copolymer micelles: implications for isoporous membrane ordering}, 
      author={Nicolas Moreno and Suzana Nunes and Victor Calo},
      year={2023},
      eprint={2304.03900},
      archivePrefix={arXiv},
      primaryClass={cond-mat.soft}
}

@misc{MorenoGeneral,
      title={Generalized Lagrangian Heterogenous Multiscale Modeling of Complex Fluids}, 
      author={Nicolas Moreno and Marco Ellero},
      year={2022},
      eprint={2211.05080},
      archivePrefix={arXiv},
      primaryClass={physics.flu-dyn}
}

@article{Texier2023, title={Shear-thickening suspensions down inclines: from Kapitza to Oobleck waves}, volume={959}, DOI={10.1017/jfm.2023.162}, journal={Journal of Fluid Mechanics}, publisher={Cambridge University Press}, author={Darbois Texier, Baptiste and Lhuissier, Henri and Metzger, Bloen and Forterre, Yoël}, year={2023}, pages={A27}}

@article{Maron,
title = {Application of ree-eyring generalized flow theory to suspensions of spherical particles},
journal = {Journal of Colloid Science},
volume = {11},
number = {1},
pages = {80-95},
year = {1956},
issn = {0095-8522},
doi = {https://doi.org/10.1016/0095-8522(56)90023-X},
url = {https://www.sciencedirect.com/science/article/pii/009585225690023X},
author = {Samuel H. Maron and Percy E. Pierce},
abstract = {The generalized flow theory of Ree and Eyring has been applied successfully to the extensive data of Maron and Fok (3) on the flow behavior of X-667 latex in both the Newtonian and non-Newtonian regions. By postulation of the presence of two flow units, a Newtonian water unit and a latex particle flow unit which may be non-Newtonian, an equation involving three parameters was obtained which reproduced very well dependence of the viscosity on rate of shear at all temperatures and concentrations. Further, the theory predicted the correct dependence of the parameters on temperature, from which could be obtained the heats of activation for flow of both the water and latex particles. Both heats of activation were found to be independent of concentration, with that of the water being the same as for the pure liquid. The theory does not predict the concentration dependence of the parameters. However, empirical equations for such dependence were deduced, from which it was possible to ascertain the values of the parameters in the Newtonian range below a volume fraction ν = 0.25, and to calculate therefrom Newtonian relative viscosities in good agreement with the observed ones at all temperatures and concentrations. Further, on extrapolation to ν = 0, νspνt was found to be 2.60 as against the expected Einstein value of 2.50 for suspensions of spheres, while extrapolation to infinite viscosity gave a volume fraction in very good agreement with that expected for the rhombohedral close packing of nonuniform spheres. From the combination of the theoretical and empirical equations were obtained also expressions for the values of the “molecular” parameters of the theory as functions of temperature and concentration, and the entropy of activation for the flow of the latex particles. The distance between equilibrium positions of the water molecules was found to vary from 13 A. to zero between ν = 0 and the volume fraction at which the viscosity becomes infinite. On the other hand, the distances between equilibrium positions and planes of latex particles varied from infinity to zero between the same concentration limits.}
}

@article{MariSeto,
  title = {Discontinuous Shear Thickening of Frictional Hard-Sphere Suspensions},
  author = {Seto, Ryohei and Mari, Romain and Morris, Jeffrey F. and Denn, Morton M.},
  journal = {Phys. Rev. Lett.},
  volume = {111},
  issue = {21},
  pages = {218301},
  numpages = {5},
  year = {2013},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.111.218301},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.218301}
}


@article{CAppelaere,
  title = {Rheology, birefringence, and small-angle neutron scattering in a charged micellar system: Evidence of a shear-induced phase transition},
  author = {Cappelaere, E. and Berret, J. F. and Decruppe, J. P. and Cressely, R. and Lindner, P.},
  journal = {Phys. Rev. E},
  volume = {56},
  issue = {2},
  pages = {1869--1878},
  numpages = {0},
  year = {1997},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.56.1869},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.56.1869}
}
 
 @Article{Britton1999,
author={Britton, M. M.
and Callaghan, P. T.},
title={Shear banding instability in wormlike micellar solutions},
journal={The European Physical Journal B - Condensed Matter and Complex Systems},
year={1999},
month={Jan},
day={01},
volume={7},
number={2},
pages={237-249},
abstract={Using NMR velocimetry and mechanical measurements we study the flow dynamics, within a cone-and-plate rheometer, of the wormlike micelle system, cetylpyridinium chloride/sodium salicylate (CPyCl/NaSal) at 100 mM/60 mM concentration in distilled water. Depending on precise conditions within the system, two classes of behaviour are observed, one in which the boundary between different shear rate phases fluctuates rapidly (on the order of tens of milliseconds) and one in which it migrates slowly with a time constant of many seconds. These modes of behaviour may depend on minor solution impurities, which presumably affect the detailed constitutive properties, but also on the externally applied shear rate within a given system. We argue that the slow migrations are governed by stress relaxation effects while the rapid migrations are flow driven and arise from interfacial instability.},
issn={1434-6036},
doi={10.1007/s100510050610},
url={https://doi.org/10.1007/s100510050610}
}



@Article{Fielding,
author ="Fielding, Suzanne M.",
title  ="Complex dynamics of shear banded flows",
journal  ="Soft Matter",
year  ="2007",
volume  ="3",
issue  ="10",
pages  ="1262-1279",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/B707980J",
url  ="http://dx.doi.org/10.1039/B707980J",
abstract  ="Many complex fluids undergo a flow induced transition to a state of coexisting bands of differing viscosities and internal structuring. This effect{,} which is called “shear banding”{,} is widely observed in wormlike micellar surfactants{,} onion surfactants{,} colloidal suspensions and polymer solutions. According to a rapidly accumulating body of experimental evidence{,} shear bands often exhibit complex dynamics{,} which can be either oscillatory or chaotic in nature. This can be seen in the unsteady response of the bulk rheological signals{,} and in the motion of the interface between the bands. After giving a brief overview of this experimental evidence{,} we review in some detail recent efforts to address it theoretically."}

@article{Olmsted,
author = {Olmsted, Peter and Radulescu, Ovidiu and Lu, C-Y},
year = {2000},
month = {03},
pages = {257-275},
title = {Johnson-Segalman model with a diffusion term in cylindrical Couette flow},
volume = {44},
journal = {Journal of Rheology - J RHEOL},
doi = {10.1122/1.551085}
}
@article{Herle,
author = {Herle, Vishweshwara and Fischer, Peter and Windhab, Erich J.},
title = {Stress Driven Shear Bands and the Effect of Confinement on Their StructuresA Rheological, Flow Visualization, and Rheo-SALS Study},
journal = {Langmuir},
volume = {21},
number = {20},
pages = {9051-9057},
year = {2005},
doi = {10.1021/la0513959},
    note ={PMID: 16171332},

URL = { 
        https://doi.org/10.1021/la0513959
    
},
eprint = { 
        https://doi.org/10.1021/la0513959
    
}

}

 @article{LIND2011,
title = {Incompressible smoothed particle hydrodynamics for free-surface flows: A generalised diffusion-based algorithm for stability and validations for impulsive flows and propagating waves},
journal = {Journal of Computational Physics},
volume = {231},
number = {4},
pages = {1499-1523},
year = {2012},
issn = {0021-9991},
doi = {https://doi.org/10.1016/j.jcp.2011.10.027},
url = {https://www.sciencedirect.com/science/article/pii/S0021999111006279},
author = {S.J. Lind and R. Xu and P.K. Stansby and B.D. Rogers},
keywords = {Incompressible SPH, Free-surface flow simulation, Fick’s law, Truncated-kernel error},
abstract = {The incompressible smoothed particle hydrodynamics (ISPH) method with projection-based pressure correction has been shown to be highly accurate and stable for internal flows and, importantly for many problems, the pressure field is virtually noise-free in contrast to the weakly compressible SPH approach (Xu et al., 2009 [31]). However for almost inviscid fluids instabilities at the free surface occur due to errors associated with the truncated kernels. A new algorithm is presented which remedies this issue, giving stable and accurate solutions to both internal and free-surface flows. Generalising the particle shifting approach of Xu et al. (2009) [31], the algorithm is based upon Fick’s law of diffusion and shifts particles in a manner that prevents highly anisotropic distributions and the onset of numerical instability. The algorithm is validated against analytical solutions for an internal flow at higher Reynolds numbers than previously, the flow due to an impulsively started plate and highly accurate solutions for wet bed dam break problems at zero and small times. The method is then validated for progressive regular waves with paddle motion defined by linear theory. The accurate predictions demonstrate the effectiveness of the algorithm in stabilising solutions and minimising the surface instabilities generated by the inevitable errors associated with truncated kernels. The test cases are thought to provide a more thorough quantitative validation than previously undertaken.}
}

@ARTICLE{Wagner2017,
       author = {{V{\'a}zquez-Quesada}, A. and {Wagner}, N.~J. and {Ellero}, M.},
        title = "{Planar channel flow of a discontinuous shear-thickening model fluid: Theory and simulation}",
      journal = {Physics of Fluids},
         year = 2017,
        month = oct,
       volume = {29},
       number = {10},
          eid = {103104},
        pages = {103104},
          doi = {10.1063/1.4997053},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017PhFl...29j3104V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Tanner2005,
title = {SPH simulations of transient viscoelastic flows at low Reynolds number},
journal = {Journal of Non-Newtonian Fluid Mechanics},
volume = {132},
number = {1},
pages = {61-72},
year = {2005},
issn = {0377-0257},
doi = {https://doi.org/10.1016/j.jnnfm.2005.08.012},
url = {https://www.sciencedirect.com/science/article/pii/S0377025705001990},
author = {M. Ellero and R.I. Tanner},
keywords = {SPH, Meshfree methods, Viscoelasticity, Transient flows, UCM fluid, Oldroyd-B fluid},
abstract = {A numerical study on the transient flow of a viscoelastic fluid is presented. The numerical framework is that of Smoothed Particle Hydrodynamics (SPH) already used by Ellero et al. in previous simulations of Non-Newtonian flows [J. Non-Newtonian Fluid. Mech. 105 (2002) 35–51]. In particular, the start-up flow between parallel plates is simulated for an Oldroyd-B and UCM fluid at low Reynolds number. Results for a Newtonian fluid are also shown for comparison. The numerical results are presented and compared with available theoretical solutions, showing a very good agreement. In particular, the simulations of an Oldroyd-B fluid have been found to be stable and accurate for a wide range of the Weissenberg number. In the case of a UCM fluid, the absence of a viscous term in the momentum equation makes its numerical modelling harder. Namely, the process is characterised by a travelling damped wave, which, if not accurately resolved, can lead to the rapid growth of small oscillations in time eventually causing divergence. On the other hand, if specifically dealing with transient flow problems, stabilising techniques such as BSD, EVSS or AVSS can not be used either; whenever used in conjunction with decoupled solution algorithms, they give an excessive oversmoothing in the results which deteriorates the final accuracy. In this work, we consider an exact SPH discretisation of the hyperbolic equation characterising the UCM model. SPH simulations are finally performed for different Weissenberg numbers showing very promising results. Finally, a discussion on the SPH treatment of the boundary conditions for general hydrodynamics problems is also outlined following the approach of ‘SPH boundary particles’ introduced by Morris for the simulations of low Reynolds number flows.}
}

@article{KALATEH202051,
title = {Simulation of cavitating fluid–Structure interaction using SPH–FE method},
journal = {Mathematics and Computers in Simulation},
volume = {173},
pages = {51-70},
year = {2020},
issn = {0378-4754},
doi = {https://doi.org/10.1016/j.matcom.2020.01.019},
url = {https://www.sciencedirect.com/science/article/pii/S0378475420300264},
author = {Farhoud Kalateh and Ali Koosheh},
keywords = {Cavitating flow, Fluid–structure interaction, Smoothed particle hydrodynamics (SPH), Finite element method (FEM), Immersed boundary, Multi-phase fluid, Phase change},
abstract = {In the present paper, a modified version of SPH–FE is proposed to study the cavitating fluid interaction with the convergent–divergent nozzle. The additional terms of mass/momentum transfer, surface tension and pressure based phase change are added to the standard SPH equations to track the growth, convection and collapse of the cavitation phenomenon. Due to using the particle-based method for the fluid, no transitional phase is defined and the certain particle phase is determined by the absolute pressure value in comparison with vapor pressure. The comparison of the results of modified SPH with those of finite volume as a grid-based method shows that the cavitating region can be accurately modeled in the convergent–divergent nozzle. Then, the interaction of cavitating fluid flow–nozzle wall is simulated by the improved SPH–FE algorithm for the different types of steel where the good agreement is obtained in comparison with the other similar numerical methods. Also, it is concluded that considering cavitation in the fluid flow can generally change the nozzle behavior slightly and increase the stress values inside its body.}
}

@Article{Reece2020,
author={Reece, Georgina
and Rogers, Benedict D.
and Lind, Steven
and Fourtakas, Georgios},
title={New instability and mixing simulations using SPH and a novel mixing measure},
journal={Journal of Hydrodynamics},
year={2020},
month={Aug},
day={01},
volume={32},
number={4},
pages={684-698},
abstract={This paper assesses the ability of smoothed particle hydrodynamics (SPH) to simulate mixing of two-phase flows and their transition to instabilities under different flow regimes. A new measure for quantification of the degree of mixing between phases in a Lagrangian framework is also developed. The method is validated using the lid-driven cavity and two-phase Poiseuille flow cases. The velocity along the centre of the cavity is compared with results from the literature, whilst commercial volume-of-fluid code STAR-CCM+ provides a benchmark for the mixing and different mixing measures are considered. The velocity of two-phase Poiseuille flow along the channel is compared to the analytical solution, and the appearance of interfacial instabilities with perturbation theory. This is the first time SPH has been used to investigate the onset and development of these instabilities. In particular, it is able to model the deforming shape of the interface, which is not given by analytical studies, while also offering improved predictions over conventional mesh-based computational fluid dynamics simulations.},
issn={1878-0342},
doi={10.1007/s42241-020-0045-x},
url={https://doi.org/10.1007/s42241-020-0045-x}
}


@article{Shimizu2016,
 title={Simulation of three-dimensional rapid free-surface granular flow past different types of obstructions using the SPH method}, volume={62}, DOI={10.1017/jog.2016.22}, number={232}, journal={Journal of Glaciology}, publisher={Cambridge University Press}, author={ABDELRAZEK, AHMED M. and KIMURA, ICHIRO and SHIMIZU, YASUYUKI}, year={2016}, pages={335–347}}
@article{Jaeger2019,
  title = {Stress Controlled Rheology of Dense Suspensions Using Transient Flows},
  author = {Han, Endao and James, Nicole M. and Jaeger, Heinrich M.},
  journal = {Phys. Rev. Lett.},
  volume = {123},
  issue = {24},
  pages = {248002},
  numpages = {6},
  year = {2019},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.123.248002},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.123.248002}
}

@article{Ozturk2020,
  title={Flow-to-fracture transition and pattern formation in a discontinuous shear thickening fluid},
  author={Deren Ozturk and Miles L. Morgan and Bj{\o}rnar Sandnes},
  journal={Communications Physics},
  year={2020},
  volume={3},
  pages={1-9}
}
@article {Peter2016,
	Title = {Direct observation of dynamic shear jamming in dense suspensions},
	Author = {Peters, Ivo R and Majumdar, Sayantan and Jaeger, Heinrich M},
	DOI = {10.1038/nature17167},
	Number = {7598},
	Volume = {532},
	Month = {April},
	Year = {2016},
	Journal = {Nature},
	ISSN = {0028-0836},
	Pages = {214—217},
	Abstract = {Liquid-like at rest, dense suspensions of hard particles can undergo striking transformations in behaviour when agitated or sheared. These phenomena include solidification during rapid impact, as well as strong shear thickening characterized by discontinuous, orders-of-magnitude increases in suspension viscosity. Much of this highly non-Newtonian behaviour has recently been interpreted within the framework of a jamming transition. However, although jamming indeed induces solid-like rigidity, even a strongly shear-thickened state still flows and thus cannot be fully jammed. Furthermore, although suspensions are incompressible, the onset of rigidity in the standard jamming scenario requires an increase in particle density. Finally, whereas shear thickening occurs in the steady state, impact-induced solidification is transient. As a result, it has remained unclear how these dense suspension phenomena are related and how they are connected to jamming. Here we resolve this by systematically exploring both the steady-state and transient regimes with the same experimental system. We demonstrate that a fully jammed, solid-like state can be reached without compression and instead purely with shear, as recently proposed for dry granular systems. This state is created by transient shear-jamming fronts, which we track directly. We also show that shear stress, rather than shear rate, is the key control parameter. From these findings we map out a state diagram with particle density and shear stress as variables. We identify discontinuous shear thickening with a marginally jammed regime just below the onset of full, solid-like jamming. This state diagram provides a unifying framework, compatible with prior experimental and simulation results on dense suspensions, that connects steady-state and transient behaviour in terms of a dynamic shear-jamming process.},
	URL = {https://doi.org/10.1038/nature17167},
}
@article{Hermes2016,
author = {Hermes,Michiel  and Guy,Ben M.  and Poon,Wilson C. K.  and Poy,Guilhem  and Cates,Michael E.  and Wyart,Matthieu },
title = {Unsteady flow and particle migration in dense, non-Brownian suspensions},
journal = {Journal of Rheology},
volume = {60},
number = {5},
pages = {905-916},
year = {2016},
doi = {10.1122/1.4953814},

URL = { 
        https://doi.org/10.1122/1.4953814
    
},
eprint = { 
        https://doi.org/10.1122/1.4953814
    
}

}

@article{Texier2020,
author = {Texier, Baptiste and Lhuissier, Henri and Forterre, Yoël and Metzger, Bloen},
year = {2020},
month = {12},
pages = {1234567890},
title = {Surface-wave instability without inertia in shear- thickening suspensions},
volume = {3},
journal = {Communications Physics},
doi = {10.1038/s42005-020-00500-4}
}
@article{Balmforth2005,
title = {Roll waves on flowing cornstarch suspensions},
journal = {Physics Letters A},
volume = {338},
number = {6},
pages = {479-484},
year = {2005},
issn = {0375-9601},
doi = {https://doi.org/10.1016/j.physleta.2005.02.071},
url = {https://www.sciencedirect.com/science/article/pii/S0375960105003257},
author = {N.J. Balmforth and J.W.M. Bush and R.V. Craster},
abstract = {We report a traveling wave instability in low Reynolds number flows of aqueous concentrated suspensions of corn starch. The experimental observations are difficult to reconcile with theoretical predictions based on simple rheological models which indicate that flows are stable at low Reynolds number.}
}
@article{Rossi2022,
title = {SPH simulations of thixo-viscoplastic fluid flow past a cylinder},
journal = {Journal of Non-Newtonian Fluid Mechanics},
volume = {308},
pages = {104891},
year = {2022},
issn = {0377-0257},
doi = {https://doi.org/10.1016/j.jnnfm.2022.104891},
url = {https://www.sciencedirect.com/science/article/pii/S0377025722001161},
author = {E. Rossi and I. {Garcia de Beristain} and A. Vazquez-Quesada and J.E. López-Aguilar and M. Ellero},
keywords = {Viscoplasticity, Thixotropy, SPH},
abstract = {Thixotropic materials are complex fluids that display time-dependent viscosity and/or yield-stress response upon the application of a fixed deformation, while recovering their original structured-state when the deformation is discontinued. Thixotropic effects are presents in many different systems and applications, ranging from food products, such as ketchup, to metals, such as molten aluminum. In this work we present a first attempt to simulate the rheological properties of thixo-viscoplastic flows using a Smoothed Particle Hydrodynamic (SPH) method. The study set up is a 2D flow around a circular cylinder as well as a simple shear flow between parallel plates to validate our numerical results. SPH solutions are compared with simulations performed using the open-source Finite Volume Method solver RheoTool, based on OpenFOAM. The viscoplastic model used in this work is the Papanastasiou model combined with a recently developed microstructural one, in order to include thixotropy. In this thixo-viscoplastic framework, we analyze the flow properties in terms of yield-fronts, streamlines and structure-parameter fields at different Bingham and Thixotropy numbers, through microstructural thixotropic and yield-stress parameters variation. Obtained results show an important novelty: an asymmetry in the thixo-viscoplastic flow around the cylinder.}
}
@article{Xu2016,
title = {An improved weakly compressible SPH method for simulating free surface flows of viscous and viscoelastic fluids},
journal = {Computer Physics Communications},
volume = {201},
pages = {43-62},
year = {2016},
issn = {0010-4655},
doi = {https://doi.org/10.1016/j.cpc.2015.12.016},
url = {https://www.sciencedirect.com/science/article/pii/S0010465515004543},
author = {Xiaoyang Xu and Xiao-Long Deng},
keywords = {Smoothed particle hydrodynamics, Free surface flow, Viscous fluid, Viscoelastic fluid},
abstract = {In this paper, an improved weakly compressible smoothed particle hydrodynamics (SPH) method is proposed to simulate transient free surface flows of viscous and viscoelastic fluids. The improved SPH algorithm includes the implementation of (i) the mixed symmetric correction of kernel gradient to improve the accuracy and stability of traditional SPH method and (ii) the Rusanov flux in the continuity equation for improving the computation of pressure distributions in the dynamics of liquids. To assess the effectiveness of the improved SPH algorithm, a number of numerical examples including the stretching of an initially circular water drop, dam breaking flow against a vertical wall, the impact of viscous and viscoelastic fluid drop with a rigid wall, and the extrudate swell of viscoelastic fluid have been presented and compared with available numerical and experimental data in literature. The convergent behavior of the improved SPH algorithm has also been studied by using different number of particles. All numerical results demonstrate that the improved SPH algorithm proposed here is capable of modeling free surface flows of viscous and viscoelastic fluids accurately and stably, and even more important, also computing an accurate and little oscillatory pressure field.}
}
@article{Ellero2012,
title = {SPH simulations of a viscoelastic flow around a periodic array of cylinders confined in a channel},
journal = {Journal of Non-Newtonian Fluid Mechanics},
volume = {167-168},
pages = {1-8},
year = {2012},
issn = {0377-0257},
doi = {https://doi.org/10.1016/j.jnnfm.2011.09.002},
url = {https://www.sciencedirect.com/science/article/pii/S0377025711002199},
author = {A. Vázquez-Quesada and M. Ellero},
keywords = {Smoothed Particle Hydrodynamics, Oldroyd-B model, Elastic instabilities},
abstract = {In this paper a numerical study on the performance of the Smoothed Particle Hydrodynamics method (SPH) in the case of a flow of a viscoelastic liquid around a linear array of cylinders confined in a channel is presented. Numerical convergence in the case of a low Reynolds number Newtonian flow was demonstrated by Ellero et al. in [Int. J. Numer. Methods Eng. 86 (2011) 1027]. Here viscoelastic effects are incorporated in the SPH scheme according to the Oldroyd-B model presented in [Phys. Rev. E 79 (2009) 056707]. Good agreement of the dimensionless drag force acting on the cylinder with literature data is observed for a wide range of Weissenberg numbers We. The case of closely spaced cylinders is also investigated and the impact of We on the solution discussed. It turns out that in this case the Newtonian solution exhibits a stable secondary flow represented by two counter-rotating vortices. When elasticity is considered, above a critical Weissenberg number Wec these vortices become unstable, breaking the plane symmetry and producing a quasi-periodic flow of mass in and out of the gap region between cylinders. Correspondingly, the flow becomes increasingly unsteady and a dramatic increase in the cylinder’s drag is observed. The results are in qualitative agreement with experimental observations made on Boger liquids under similar flow conditions.}
}
@article{Liu2012,
  title={SPH simulations of three-dimensional non-Newtonian free surface flows},
  author={Xiaoyang Xu and Jie Ouyang and Bin-Xin Yang and Zhijun Liu},
  journal={Computer Methods in Applied Mechanics and Engineering},
  year={2013},
  volume={256},
  pages={101-116}
}
@article{Hosseini2007,
title = {An incompressible SPH method for simulation of unsteady viscoelastic free-surface flows},
journal = {International Journal of Non-Linear Mechanics},
volume = {42},
number = {10},
pages = {1210-1223},
year = {2007},
issn = {0020-7462},
doi = {https://doi.org/10.1016/j.ijnonlinmec.2007.09.006},
url = {https://www.sciencedirect.com/science/article/pii/S0020746207001862},
author = {A. Rafiee and M.T. Manzari and M. Hosseini},
keywords = {Smoothed particle hydrodynamics, Viscoelastic, Artificial stress, Free surface},
abstract = {In this paper, an incompressible smoothed particle hydrodynamics (SPH) method is presented to solve unsteady free-surface flows. Both Newtonian and viscoelastic fluids are considered. In the case of viscoelastic fluids, both the Maxwell and Oldroyd-B models are investigated. The proposed SPH method uses a Poisson pressure equation to satisfy the incompressibility constraints. The solution algorithm is an explicit predictor-corrector scheme and employs an adaptive smoothing length based on density variations. To alleviate the numerical difficulties encountered when fluid is highly stretched, an artificial stress term is incorporated into the momentum equation which reduces the risk of unrealistic fractures in the material. Two challenging test cases, the impacting drop and the jet buckling problems, are solved to demonstrate the capability of the proposed scheme in handling viscoelastic flows with complex free surfaces. The jet buckling test case was solved for a wide range of Weissenberg numbers. It was shown that in all cases the method is stable and fairly accurate and agrees well with the available data.}
}
@article{Fang2009,
title = {Improved SPH methods for simulating free surface flows of viscous fluids},
journal = {Applied Numerical Mathematics},
volume = {59},
number = {2},
pages = {251-271},
year = {2009},
issn = {0168-9274},
doi = {https://doi.org/10.1016/j.apnum.2008.02.003},
url = {https://www.sciencedirect.com/science/article/pii/S0168927408000305},
author = {Jiannong Fang and Aurèle Parriaux and Martin Rentschler and Christophe Ancey},
keywords = {Meshless/meshfree method, Smoothed Particle Hydrodynamics, Finite particle method, Viscous fluids, Free surface flows},
abstract = {In this paper we present two enhanced variants of the smoothed particle hydrodynamics (SPH) method for the numerical simulation of free surface flows of viscous fluids. Improvements are achieved by deriving a new set of general discrete SPH-like equations under an energy-based framework and applying a corrected (high-order) or coupled particle approximation scheme for function derivatives. By doing so, we ensure that the enhanced variants retain the conservative nature of SPH which is important for the stability of long-term simulations. Among various corrected approximations, we here implement the one obtained by the so-called finite particle method (FPM) within the framework to produce a higher-order SPH method which conserves both linear and angular momentums. In order to improve the efficiency of the higher-order variant, a coupled approach with the idea of using the SPH approximation for the interior particles and the FPM approximation for the exterior particles is also proposed and tested in this paper. Three prototype tests concerning free deformation of a viscous fluid patch with free surface are presented with comparisons between different methods to demonstrate the performance of the two proposed methods. Numerical results show that both the higher-order version using FPM and the coupled version using FPM/SPH outperform the original version of SPH in respect of accuracy and stability.}
}
@article{Fang2006,
  title={A numerical study of the SPH method for simulating transient viscoelastic free surface flows},
  author={Jiannong Fang and Robert G. Owens and Laurent Tacher and Aur{\`e}le Parriaux},
  journal={Journal of Non-newtonian Fluid Mechanics},
  year={2006},
  volume={139},
  pages={68-84}
}
@article{Ellero2002,
title = {Viscoelastic flows studied by smoothed particle dynamics},
journal = {Journal of Non-Newtonian Fluid Mechanics},
volume = {105},
number = {1},
pages = {35-51},
year = {2002},
issn = {0377-0257},
doi = {https://doi.org/10.1016/S0377-0257(02)00059-9},
url = {https://www.sciencedirect.com/science/article/pii/S0377025702000599},
author = {Marco Ellero and Martin Kröger and Siegfried Hess},
keywords = {Smoothed particle hydrodynamics, Viscoelasticity, Isothermal flow, Fluid-pseudo-particles, Jaumann–Maxwell model},
abstract = {A viscoelastic numerical scheme based on smoothed particle dynamics is presented. The concept goes a step beyond smoothed particle hydrodynamics (SPH) which is a grid-free Lagrangian method describing the flow by fluid-pseudo-particles. The relevant properties are interpolated directly on the resulting movable grid. In this work, the effect of viscoelasticity is incorporated into the ordinary conservation laws by a differential constitutive equation supplied for the stress tensor. In order to give confidence in the methodology we explicitly consider the non-stationary simple corotational Maxwell model in a channel geometry. Without further developments the scheme is applicable to ‘realistic’ models relevant for three-dimensional (3D) viscoelastic flows in complex geometries.}
}
@article{Monaghan2005,
doi = {10.1088/0034-4885/68/8/R01},
url = {https://dx.doi.org/10.1088/0034-4885/68/8/R01},
year = {2005},
month = {jul},
publisher = {},
volume = {68},
number = {8},
pages = {1703},
author = {J J Monaghan},
title = {Smoothed particle hydrodynamics},
journal = {Reports on Progress in Physics},
abstract = {In this review the theory and application of Smoothed particle hydrodynamics (SPH) since its inception in 1977 are discussed. Emphasis is placed on the strengths and weaknesses, the analogy with particle dynamics and the numerous areas where SPH has been successfully applied.}
}
@article{Monaghan1977,
    author = {Gingold, R. A. and Monaghan, J. J.},
    title = "{Smoothed particle hydrodynamics: theory and application to non-spherical stars}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {181},
    number = {3},
    pages = {375-389},
    year = {1977},
    month = {12},
    abstract = "{A new hydrodynamic code applicable to a space of an arbitrary number of dimensions is discussed and applied to a variety of polytropic stellar models. The principal feature of the method is the use of statistical techniques to recover analytical expressions for the physical variables from a known distribution of fluid elements. The equations of motion take the form of Newtonian equations for particles. Starting with a non-axisymmetric distribution of approximately 80 particles in three dimensions, the method is found to reproduce the structure of uniformly rotating and magnetic polytropes to within a few per cent. The method may be easily extended to deal with more complicated physical models.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/181.3.375},
    url = {https://doi.org/10.1093/mnras/181.3.375},
    eprint = {https://academic.oup.com/mnras/article-pdf/181/3/375/3104055/mnras181-0375.pdf},
}

@ARTICLE{Lucy1977,
    author = {{Lucy}, L.~B.},
    title = "{A numerical approach to the testing of the fission hypothesis.}",
    journal = {Astronomical Journal},
    keywords = {Binary Stars, Hypotheses, Nuclear Fission, Numerical Analysis, Protostars, Stellar Evolution, Astronomical Models, Difference Equations, Gas Dynamics, Monte Carlo Method, Numerical Stability, Particle Motion, Stellar Rotation, Astrophysics},
    year = 1977,
    Month = Dec,
    volume = {82},
    pages = {1013--1024},
    doi = {10.1086/112164},
   adsurl = {https://ui.adsabs.harvard.edu/abs/1977AJ.....82.1013L},
   adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Lind2020,
author = {Lind, Steven J.  and Rogers, Benedict D.  and Stansby, Peter K. },
title = {Review of smoothed particle hydrodynamics: towards converged Lagrangian flow modelling},
journal = {Proceedings of the Royal Society A: Mathematical, Physical and Engineering Sciences},
volume = {476},
number = {2241},
pages = {20190801},
year = {2020},
doi = {10.1098/rspa.2019.0801},
URL = {https://royalsocietypublishing.org/doi/abs/10.1098/rspa.2019.0801},
eprint = {https://royalsocietypublishing.org/doi/pdf/10.1098/rspa.2019.0801}
,
    abstract = { This paper presents a review of the progress of smoothed particle hydrodynamics (SPH) towards high-order converged simulations. As a mesh-free Lagrangian method suitable for complex flows with interfaces and multiple phases, SPH has developed considerably in the past decade. While original applications were in astrophysics, early engineering applications showed the versatility and robustness of the method without emphasis on accuracy and convergence. The early method was of weakly compressible form resulting in noisy pressures due to spurious pressure waves. This was effectively removed in the incompressible (divergence-free) form which followed; since then the weakly compressible form has been advanced, reducing pressure noise. Now numerical convergence studies are standard. While the method is computationally demanding on conventional processors, it is well suited to parallel processing on massively parallel computing and graphics processing units. Applications are diverse and encompass wave–structure interaction, geophysical flows due to landslides, nuclear sludge flows, welding, gearbox flows and many others. In the state of the art, convergence is typically between the first- and second-order theoretical limits. Recent advances are improving convergence to fourth order (and higher) and these will also be outlined. This can be necessary to resolve multi-scale aspects of turbulent flow. }
}
@article{WilsonCates2019,
  title = {Constitutive Model for Time-Dependent Flows of Shear-Thickening Suspensions},
  author = {Gillissen, J. J. J. and Ness, C. and Peterson, J. D. and Wilson, H. J. and Cates, M. E.},
  journal = {Phys. Rev. Lett.},
  volume = {123},
  issue = {21},
  pages = {214504},
  numpages = {6},
  year = {2019},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.123.214504},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.123.214504}
}

@article{WilsonCates2020,
author = {Gillissen,J. J. J.  and Ness,C.  and Peterson,J. D.  and Wilson,H. J.  and Cates,M. E. },
title = {Constitutive model for shear-thickening suspensions: Predictions for steady shear with superposed transverse oscillations},
journal = {Journal of Rheology},
volume = {64},
number = {2},
pages = {353-365},
year = {2020},
doi = {10.1122/1.5129657},

URL = { 
        https://doi.org/10.1122/1.5129657
    
},
eprint = { 
        https://doi.org/10.1122/1.5129657
    
}

}
@article{Kamrin2019,
author = {Aaron S. Baumgarten and Ken Kamrin },
title = {A general constitutive model for dense, fine-particle suspensions validated in many geometries},
journal = {Proceedings of the National Academy of Sciences},
volume = {116},
number = {42},
pages = {20828-20836},
year = {2019},
doi = {10.1073/pnas.1908065116},
URL = {https://www.pnas.org/doi/abs/10.1073/pnas.1908065116},
eprint = {https://www.pnas.org/doi/pdf/10.1073/pnas.1908065116},
abstract = {Fine-particle suspensions (such as cornstarch mixed with water) exhibit dramatic changes in viscosity when sheared, producing fascinating behaviors that captivate children and rheologists alike. Examination of these mixtures in simple flow geometries suggests intergranular repulsion and its influence on the frictional nature of granular contacts is central to this effect—for mixtures at rest or shearing slowly, repulsion prevents frictional contacts from forming between particles, whereas when sheared more forcefully, granular stresses overcome the repulsion allowing particles to interact frictionally and form microscopic structures that resist flow. Previous constitutive studies of these mixtures have focused on particular cases, typically limited to 2D, steady, simple shearing flows. In this work, we introduce a predictive and general, 3D continuum model for this material, using mixture theory to couple the fluid and particle phases. Playing a central role in the model, we introduce a microstructural state variable, whose evolution is deduced from small-scale physical arguments and checked with existing data. Our space- and time-dependent model is implemented numerically in a variety of unsteady, nonuniform flow configurations where it is shown to accurately capture a variety of key behaviors: 1) the continuous shear-thickening (CST) and discontinuous shear-thickening (DST) behavior observed in steady flows, 2) the time-dependent propagation of “shear jamming fronts,” 3) the time-dependent propagation of “impact-activated jamming fronts,” and 4) the non-Newtonian, “running on oobleck” effect, wherein fast locomotors stay afloat while slow ones sink.}}


@article{WC2014,
  title = {Discontinuous Shear Thickening without Inertia in Dense Non-Brownian Suspensions},
  author = {Wyart, M. and Cates, M. E.},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  issue = {9},
  pages = {098302},
  numpages = {5},
  year = {2014},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.098302},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.098302}
}

@article{Brown_2014,
doi = {10.1088/0034-4885/77/4/046602},
url = {https://dx.doi.org/10.1088/0034-4885/77/4/046602},
year = {2014},
month = {apr},
publisher = {IOP Publishing},
volume = {77},
number = {4},
pages = {046602},
author = {Eric Brown and Heinrich M Jaeger},
title = {Shear thickening in concentrated suspensions: phenomenology, mechanisms and relations to jamming},
journal = {Reports on Progress in Physics},
abstract = {Shear thickening is a type of non-Newtonian behavior in which the stress required to shear a fluid increases faster than linearly with shear rate. Many concentrated suspensions of particles exhibit an especially dramatic version, known as Discontinuous Shear Thickening (DST), in which the stress suddenly jumps with increasing shear rate and produces solid-like behavior. The best known example of such counter-intuitive response to applied stresses occurs in mixtures of cornstarch in water. Over the last several years, this shear-induced solid-like behavior together with a variety of other unusual fluid phenomena has generated considerable interest in the physics of densely packed suspensions. In this review, we discuss the common physical properties of systems exhibiting shear thickening, and different mechanisms and models proposed to describe it. We then suggest how these mechanisms may be related and generalized, and propose a general phase diagram for shear thickening systems. We also discuss how recent work has related the physics of shear thickening to that of granular materials and jammed systems. Since DST is described by models that require only simple generic interactions between particles, we outline the broader context of other concentrated many-particle systems such as foams and emulsions, and explain why DST is restricted to the parameter regime of hard-particle suspensions. Finally, we discuss some of the outstanding problems and emerging opportunities.}
}

@article{lind2021,
title = {Incompressible smoothed particle hydrodynamics for free-surface flows: A generalised diffusion-based algorithm for stability and validations for impulsive flows and propagating waves},
journal = {Journal of Computational Physics},
volume = {231},
number = {4},
pages = {1499-1523},
year = {2012},
issn = {0021-9991},
doi = {https://doi.org/10.1016/j.jcp.2011.10.027},
url = {https://www.sciencedirect.com/science/article/pii/S0021999111006279},
author = {S.J. Lind and R. Xu and P.K. Stansby and B.D. Rogers},
keywords = {Incompressible SPH, Free-surface flow simulation, Fick’s law, Truncated-kernel error},
abstract = {The incompressible smoothed particle hydrodynamics (ISPH) method with projection-based pressure correction has been shown to be highly accurate and stable for internal flows and, importantly for many problems, the pressure field is virtually noise-free in contrast to the weakly compressible SPH approach (Xu et al., 2009 [31]). However for almost inviscid fluids instabilities at the free surface occur due to errors associated with the truncated kernels. A new algorithm is presented which remedies this issue, giving stable and accurate solutions to both internal and free-surface flows. Generalising the particle shifting approach of Xu et al. (2009) [31], the algorithm is based upon Fick’s law of diffusion and shifts particles in a manner that prevents highly anisotropic distributions and the onset of numerical instability. The algorithm is validated against analytical solutions for an internal flow at higher Reynolds numbers than previously, the flow due to an impulsively started plate and highly accurate solutions for wet bed dam break problems at zero and small times. The method is then validated for progressive regular waves with paddle motion defined by linear theory. The accurate predictions demonstrate the effectiveness of the algorithm in stabilising solutions and minimising the surface instabilities generated by the inevitable errors associated with truncated kernels. The test cases are thought to provide a more thorough quantitative validation than previously undertaken.}
}

@article{Adami2012,
title = {A generalized wall boundary condition for smoothed particle hydrodynamics},
journal = {Journal of Computational Physics},
volume = {231},
number = {21},
pages = {7057-7075},
year = {2012},
issn = {0021-9991},
doi = {https://doi.org/10.1016/j.jcp.2012.05.005},
url = {https://www.sciencedirect.com/science/article/pii/S002199911200229X},
author = {S. Adami and X.Y. Hu and N.A. Adams},
keywords = {Boundary condition, SPH, Solid walls},
abstract = {In this paper we present a new formulation of the boundary condition at static and moving solid walls in SPH simulations. Our general approach is both applicable to two and three dimensions and is very simple compared to previous wall boundary formulations. Based on a local force balance between wall and fluid particles we apply a pressure boundary condition on the solid particles to prevent wall penetration. This method can handle sharp corners and complex geometries as is demonstrated with several examples. A validation shows that we recover hydrostatic equilibrium conditions in a static tank, and a comparison of the classical dam break simulation with state-of-the-art results in literature shows good agreement. We simulate various problems such as the flow around a cylinder and the backward facing step at Re=100 to demonstrate the general applicability of this new method.}
}

@article{wagner_dst,
author = {Cwalina,Colin D.  and Wagner,Norman J. },
title = {Rheology of non-{B}rownian particles suspended in concentrated colloidal dispersions at low particle {R}eynolds number},
journal = {Journal of Rheology},
volume = {60},
number = {1},
pages = {47-59},
year = {2016},
doi = {10.1122/1.4935445},
URL = {https://doi.org/10.1122/1.4935445},
eprint = {https://doi.org/10.1122/1.4935445}
}

@article{Seto2013,
  title = {Discontinuous Shear Thickening of Frictional Hard-Sphere Suspensions},
  author = {Seto, Ryohei and Mari, Romain and Morris, Jeffrey F. and Denn, Morton M.},
  journal = {Phys. Rev. Lett.},
  volume = {111},
  issue = {21},
  pages = {218301},
  numpages = {5},
  year = {2013},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.111.218301},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.218301}
}


@article{Mari2014,
author = {Mari,Romain  and Seto,Ryohei  and Morris,Jeffrey F.  and Denn,Morton M. },
title = {Shear thickening, frictionless and frictional rheologies in non-{B}rownian           suspensions},
journal = {Journal of Rheology},
volume = {58},
number = {6},
pages = {1693-1724},
year = {2014},
doi = {10.1122/1.4890747},
URL = {https://doi.org/10.1122/1.4890747},
eprint = {https://doi.org/10.1122/1.4890747}
}

@article{Trask19,
title = "A spatially adaptive high-order meshless method for fluid-structure interactions",
journal = "Computer Methods in Applied Mechanics and Engineering",
volume = "355",
pages = "67 - 93",
year = "2019",
issn = "0045-7825",
doi = "https://doi.org/10.1016/j.cma.2019.06.009",
url = "http://www.sciencedirect.com/science/article/pii/S0045782519303494",
author = "Wei Hu and Nathaniel Trask and Xiaozhe Hu and Wenxiao Pan",
}
@article{Trask18,
title = "A compatible high-order meshless method for the {S}tokes equations with applications to suspension flows",
journal = "Journal of Computational Physics",
volume = "355",
pages = "310 - 326",
year = "2018",
issn = "0021-9991",
doi = "https://doi.org/10.1016/j.jcp.2017.10.039",
url = "http://www.sciencedirect.com/science/article/pii/S0021999117308069",
author = "Nathaniel Trask and Martin Maxey and Xiaozhe Hu",
}

@article{Trask15,
title = "A scalable consistent second-order {SPH} solver for unsteady low {R}eynolds number flows",
journal = "Computer Methods in Applied Mechanics and Engineering",
volume = "289",
pages = "155 - 178",
year = "2015",
issn = "0045-7825",
doi = "https://doi.org/10.1016/j.cma.2014.12.027",
url = "http://www.sciencedirect.com/science/article/pii/S0045782514005064",
author = "Nathaniel Trask and Martin Maxey and Kyungjoo Kim and Mauro Perego and Michael L. Parks and Kai Yang and Jinchao Xu",
}


@article{ball1997,
doi	= {10.1016/s0378-4371(97)00412-3},
title	= {A simulation technique for many spheres in quasi-static motion under frame-invariant pair drag and {B}rownian forces},
author	= {Ball, R. C. and Melrose, J. R.},
publisher	= {Elsevier Science},
journal	= {Physica A: Statistical Mechanics and its Applications},
issnp	= {0378-4371},
year	= {1997},
volume	= {247},
issue	= {1-4},
page	= {444--472},
url =       {http://gen.lib.rus.ec/scimag/index.php?s=10.1016/s0378-4371(97)00412-3},
}
@article{yamamoto1995,
author = {Yamamoto,Satoru  and Matsuoka,Takaaki},
title = {Dynamic simulation of fiber suspensions in shear flow},
journal = {The Journal of Chemical Physics},
volume = {102},
number = {5},
pages = {2254-2260},
year = {1995},
doi = {10.1063/1.468746},
URL = {https://doi.org/10.1063/1.468746},
eprint = {https://doi.org/10.1063/1.468746},
}
@article{adolfo2016_1,
author = {V{\'a}zquez-Quesada,A.  and Ellero,M. },
title = {Analytical solution for the lubrication force between two spheres in a bi-viscous fluid},
journal = {Physics of Fluids},
volume = {28},
number = {7},
pages = {073101},
year = {2016},
doi = {10.1063/1.4954815},
URL = {https://aip.scitation.org/doi/abs/10.1063/1.4954815},
eprint = {https://aip.scitation.org/doi/pdf/10.1063/1.4954815},
}
@article{adolfo2016_2,
title = "Rheology and microstructure of non-colloidal suspensions under shear studied with {S}moothed {P}article {H}ydrodynamics",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "233",
pages = "37 - 47",
year = "2016",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2015.12.009",
url = "http://www.sciencedirect.com/science/article/pii/S0377025715002189",
author = "Adolfo V{\'a}zquez-Quesada and Marco Ellero",
}
@article{sierou2002,
author = {Sierou, A.  and Brady,J. F.},
title = {Rheology and microstructure in concentrated noncolloidal suspensions},
journal = {Journal of Rheology},
volume = {46},
number = {5},
pages = {1031-1056},
year = {2002},
doi = {10.1122/1.1501925},
URL = {https://doi.org/10.1122/1.1501925},
eprint = {https://doi.org/10.1122/1.1501925}
}
@Article{bertevas2009,
author="Bertevas, Erwan and Fan, Xijun and Tanner, Roger I.",
title="Simulation of the rheological properties of suspensions of oblate spheroidal particles in a {N}ewtonian fluid",
journal="Rheologica Acta",
year="2009",
month="Oct",
day="10",
volume="49",
number="1",
pages="53",
issn="1435-1528",
doi="10.1007/s00397-009-0390-8",
url="https://doi.org/10.1007/s00397-009-0390-8"
}
@article{dAvino2007,
author = "G. D’Avino and P.L. Maffettone and M.A. Hulsen and G.W.M. Peters",
title = "A numerical method for simulating concentrated rigid particle suspensions in an elongational flow using a fixed grid",
journal = "Journal of Computational Physics",
volume = "226",
number = "1",
pages = "688 - 711",
year = "2007",
issn = "0021-9991",
doi = "https://doi.org/10.1016/j.jcp.2007.04.027",
url = "http://www.sciencedirect.com/science/article/pii/S0021999107002021",
}
@article{sierou_2001, 
title={Accelerated {S}tokesian {D}ynamics simulations}, 
volume={448}, 
DOI={10.1017/S0022112001005912}, 
journal={Journal of Fluid Mechanics}, 
publisher={Cambridge University Press}, 
author={Sierou, Asimina and Brady, John F.}, 
year={2001}, 
pages={115–146}
}
@Article{Ladd2001,
author="Ladd, A. J. C. and Verberg, R.",
title="Lattice-{B}oltzmann Simulations of Particle-Fluid Suspensions",
journal="Journal of Statistical Physics",
year="2001",
month="Sep",
day="01",
volume="104",
number="5",
pages="1191--1251",
issn="1572-9613",
doi="10.1023/A:1010414013942",
url="https://doi.org/10.1023/A:1010414013942"
}
@article{Martys2005,
author = {Martys,Nicos S. },
title = {Study of a dissipative particle dynamics based approach for modeling suspensions},
journal = {Journal of Rheology},
volume = {49},
number = {2},
pages = {401-424},
year = {2005},
doi = {10.1122/1.1849187},
URL = {https://doi.org/10.1122/1.1849187},
eprint = {https://doi.org/10.1122/1.1849187}
}
@Article{adolfo2016_3,
author="V{\'a}zquez-Quesada, Adolfo and Bian, Xin and Ellero, Marco",
title="Three-dimensional simulations of dilute and concentrated suspensions using smoothed particle hydrodynamics",
journal="Computational Particle Mechanics",
year="2016",
month="Apr",
day="01",
volume="3",
number="2",
pages="167--178",
issn="2196-4386",
doi="10.1007/s40571-015-0072-5",
url="https://doi.org/10.1007/s40571-015-0072-5"
}
@article{coussot2014,
title = "Yield stress fluid flows: {A} review of experimental data",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "211",
pages = "31 - 49",
year = "2014",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2014.05.006",
url = "http://www.sciencedirect.com/science/article/pii/S0377025714000895",
author = "P. Coussot",
}
@article{barnes1999,
title = "The yield stress - a review or {`}{$\pi$}{$\alpha$}{$\nu$}{$\tau$}{$\alpha$}~{$\rho$}{$\epsilon$}{$\iota$}{'} - everything flows?",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "81",
number = "1",
pages = "133 - 178",
year = "1999",
issn = "0377-0257",
doi = "https://doi.org/10.1016/S0377-0257(98)00094-9",
url = "http://www.sciencedirect.com/science/article/pii/S0377025798000949",
author = "Howard A. Barnes",
}
@book{larson1999,
  title={The Structure and Rheology of Complex Fluids},
  author={Larson, R.G. and Larson, R.G.},
  isbn={9780195121971},
  lccn={98019940},
  series={Topics in Chemical Engineering},
  url={https://books.google.es/books?id=Vt9fw\_pf1LUC},
  year={1999},
  publisher={OUP USA}
}
@article{ovarlez2015,
author = {Ovarlez,Guillaume  and Mahaut,Fabien  and Deboeuf,Stéphanie  and Lenoir,Nicolas  and Hormozi,Sarah  and Chateau,Xavier },
title = {Flows of suspensions of particles in yield stress fluids},
journal = {Journal of Rheology},
volume = {59},
number = {6},
pages = {1449-1486},
year = {2015},
doi = {10.1122/1.4934363},
URL = {https://doi.org/10.1122/1.4934363},
eprint = {https://doi.org/10.1122/1.4934363}
}
@article{mahaut2008,
author = {Mahaut,Fabien  and Chateau,Xavier and Coussot,Philippe  and Ovarlez,Guillaume},
title = {Yield stress and elastic modulus of suspensions of noncolloidal particles in yield stress fluids},
journal = {Journal of Rheology},
volume = {52},
number = {1},
pages = {287-313},
year = {2008},
doi = {10.1122/1.2798234},
URL = {https://doi.org/10.1122/1.2798234},
eprint = {https://doi.org/10.1122/1.2798234}
}
@article{ancey2001,
author = {Ancey,Christophe  and Jorrot,Hélène },
title = {Yield stress for particle suspensions within a clay dispersion},
journal = {Journal of Rheology},
volume = {45},
number = {2},
pages = {297-319},
year = {2001},
doi = {10.1122/1.1343879},
URL = {https://doi.org/10.1122/1.1343879},
eprint = {https://doi.org/10.1122/1.1343879}
}
@article{simon2015, 
title={Rheology of dense suspensions of non-colloidal spheres in yield-stress fluids}, 
volume={776}, 
DOI={10.1017/jfm.2015.329}, 
journal={Journal of Fluid Mechanics}, 
publisher={Cambridge University Press}, 
author={Dagois-Bohy, Simon and Hormozi, Sarah and Guazzelli, Élisabeth and Pouliquen, Olivier},
year={2015}, 
pages={R2}
}
@ARTICLE{geiker2002,
author={Geiker, M.R. and Brandl, M. and Thrane, L.N. and Nielsen, L.F.},
title={On the effect of coarse aggregate fraction and shape on the rheological properties of self-compacting concrete},
journal={Cement, Concrete and Aggregates},
year={2002},
volume={24},
number={1},
pages={3-6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-0039490208&partnerID=40&md5=614019d3cc8048f209cff0ce429b407f},
}

@Article{sengun1989_1,
author="Sengun, M. Z. and Probstein, R. F.",
title="Bimodal model of slurry viscosity with application to coal-slurries. {P}art 1. {T}heory and experiment",
journal="Rheologica Acta",
year="1989",
month="Sep",
day="01",
volume="28",
number="5",
pages="382-393",
issn="1435-1528",
doi="10.1007/BF01336805",
url="https://doi.org/10.1007/BF01336805"
}
@Article{sengun1989_2,
author="Sengun, M. Z. and Probstein, R. F.",
title="Bimodal model of slurry viscosity with application to coal-slurries. {P}art 2. {H}igh shear limit behavior",
journal="Rheologica Acta",
year="1989",
month="Sep",
day="01",
volume="28",
number="5",
pages="394--401",
issn="1435-1528",
doi="10.1007/BF01336806",
url="https://doi.org/10.1007/BF01336806"
}

@article{cohen2007,
  title = {Rigidity {P}ercolation in {P}article-{L}aden {F}oams},
  author = {Cohen-Addad, Sylvie and Krzan, Marcel and H\"ohler, Reinhard and Herzhaft, Benjamin},
  journal = {Phys. Rev. Lett.},
  volume = {99},
  issue = {16},
  pages = {168001},
  numpages = {4},
  year = {2007},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.99.168001},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.99.168001}
}

@article{firouznia2018,
title = "The interaction of two spherical particles in simple-shear flows of yield stress fluids",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "255",
pages = "19 - 38",
year = "2018",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2018.03.006",
url = "http://www.sciencedirect.com/science/article/pii/S0377025717304548",
author = "Mohammadhossein Firouznia and Bloen Metzger and Guillaume Ovarlez and Sarah Hormozi",
}

@article{deboeuf2018,
author = {Deboeuf,S.  and Lenoir,N.  and Hautemayou,D.  and Bornert,M.  and Blanc,F.  and Ovarlez,G. },
title = {Imaging non-{B}rownian particle suspensions with {X}-ray tomography: {A}pplication to the microstructure of {N}ewtonian and viscoplastic suspensions},
journal = {Journal of Rheology},
volume = {62},
number = {2},
pages = {643-663},
year = {2018},
doi = {10.1122/1.4994081},
URL = {https://doi.org/10.1122/1.4994081},
eprint = {https://doi.org/10.1122/1.4994081}
}

@article{rezea2016,
title = "Macroscopic rheological behavior of suspensions of soft solid particles in yield stress fluids",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "234",
pages = "139 - 161",
year = "2016",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2016.05.005",
url = "http://www.sciencedirect.com/science/article/pii/S037702571630060X",
author = "Reza Avazmohammadi and Pedro Ponte Castañeda",
}

@article{maleki2015, title={Macro-size drop encapsulation}, volume={769}, DOI={10.1017/jfm.2015.81}, journal={Journal of Fluid Mechanics}, publisher={Cambridge University Press}, author={Maleki, A. and Hormozi, S. and Roustaei, A. and Frigaard, I. A.}, year={2015}, pages={482–521}}

@article{ducloue2015,
title = "Rheological behaviour of suspensions of bubbles in yield stress fluids",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "215",
pages = "31 - 39",
year = "2015",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2014.10.003",
url = "http://www.sciencedirect.com/science/article/pii/S0377025714001918",
author = "Lucie Duclou{\'e} and Olivier Pitois and Julie Goyon and Xavier Chateau and Guillaume Ovarlez",
}

@Article{kogan2013,
author="Kogan, Michael and Duclou{\'e}, Lucie and Goyon, Julie and Chateau, Xavier and Pitois, Olivier
and Ovarlez, Guillaume",
title="Mixtures of foam and paste: suspensions of bubbles in yield stress fluids",
journal="Rheologica Acta",
year="2013",
month="Mar",
day="01",
volume="52",
number="3",
pages="237--253",
issn="1435-1528",
doi="10.1007/s00397-013-0677-7",
url="https://doi.org/10.1007/s00397-013-0677-7"
}

@article{ovarlez2012,
title = "Shear-induced sedimentation in yield stress fluids",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "177-178",
pages = "19 - 28",
year = "2012",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2012.03.013",
url = "http://www.sciencedirect.com/science/article/pii/S0377025712000663",
author = "Guillaume Ovarlez and François Bertrand and Philippe Coussot and Xavier Chateau",
}

@article{vu2010,
author = {Vu,Thai-Son  and Ovarlez,Guillaume  and Chateau,Xavier },
title = {Macroscopic behavior of bidisperse suspensions of noncolloidal particles in yield stress fluids},
journal = {Journal of Rheology},
volume = {54},
number = {4},
pages = {815-833},
year = {2010},
doi = {10.1122/1.3439731},
URL = {https://doi.org/10.1122/1.3439731},
eprint = {https://doi.org/10.1122/1.3439731}
}
@article{avazmohammadi2016,
title = "Macroscopic rheological behavior of suspensions of soft solid particles in yield stress fluids",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "234",
pages = "139 - 161",
year = "2016",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2016.05.005",
url = "http://www.sciencedirect.com/science/article/pii/S037702571630060X",
author = "Reza Avazmohammadi and Pedro Ponte Castañeda",
}

@article{beris1985, title={Creeping motion of a sphere through a {B}ingham plastic}, volume={158}, DOI={10.1017/S0022112085002622}, journal={Journal of Fluid Mechanics}, publisher={Cambridge University Press}, author={Beris, A. N. and Tsamopoulos, J. A. and Armstrong, R. C. and Brown, R. A.}, year={1985}, pages={219–244}}

@article{ovarlez2012,
title = "Shear-induced sedimentation in yield stress fluids",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "177-178",
pages = "19 - 28",
year = "2012",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2012.03.013",
url = "http://www.sciencedirect.com/science/article/pii/S0377025712000663",
author = "Guillaume Ovarlez and François Bertrand and Philippe Coussot and Xavier Chateau",
}

@Article{fraggedakis2016,
author ="Fraggedakis, D. and Dimakopoulos, Y. and Tsamopoulos, J.",
title  ="Yielding the yield-stress analysis: a study focused on the effects of elasticity on the settling of a single spherical particle in simple yield-stress fluids",
journal  ="Soft Matter",
year  ="2016",
volume  ="12",
issue  ="24",
pages  ="5378-5401",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C6SM00480F",
url  ="http://dx.doi.org/10.1039/C6SM00480F",
}

@article{blackery1997,
title = "Creeping motion of a sphere in tubes filled with a {B}ingham plastic material",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "70",
number = "1",
pages = "59 - 77",
year = "1997",
issn = "0377-0257",
doi = "https://doi.org/10.1016/S0377-0257(96)01536-4",
url = "http://www.sciencedirect.com/science/article/pii/S0377025796015364",
author = "Blackery, J. and Mitsoulis, E.",
}

@article{liu2002,
title = "Convergence of a regularization method for creeping flow of a {B}ingham material about a rigid sphere",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "102",
number = "2",
pages = "179 - 191",
year = "2002",
issn = "0377-0257",
doi = "https://doi.org/10.1016/S0377-0257(01)00177-X",
url = "http://www.sciencedirect.com/science/article/pii/S037702570100177X",
author = "Benjamin T Liu and Susan J Muller and Morton M Denn",
}

@article{liu2003,
title = "Interactions of two rigid spheres translating collinearly in creeping flow in a {B}ingham material",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "113",
number = "1",
pages = "49 - 67",
year = "2003",
issn = "0377-0257",
doi = "https://doi.org/10.1016/S0377-0257(03)00111-3",
url = "http://www.sciencedirect.com/science/article/pii/S0377025703001113",
author = "Benjamin T. Liu and Susan J. Muller and Morton M. Denn",
}

@article{yu2007,
title = "A fictitious domain method for dynamic simulation of particle sedimentation in {B}ingham fluids",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "145",
number = "2",
pages = "78 - 91",
year = "2007",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2007.02.007",
url = "http://www.sciencedirect.com/science/article/pii/S0377025707000663",
author = "Zhaosheng Yu and Anthony Wachs",
}

@article{glowinski1999,
title = "A distributed {L}agrange multiplier/fictitious domain method for particulate flows",
journal = "International Journal of Multiphase Flow",
volume = "25",
number = "5",
pages = "755 - 794",
year = "1999",
issn = "0301-9322",
doi = "https://doi.org/10.1016/S0301-9322(98)00048-2",
url = "http://www.sciencedirect.com/science/article/pii/S0301932298000482",
author = "R. Glowinski and T.-W. Pan and T.I. Hesla and D.D. Joseph",
}

@article{YU2006126,
title = "Numerical simulation of particle sedimentation in shear-thinning fluids with a fictitious domain method",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "136",
number = "2",
pages = "126 - 139",
year = "2006",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2006.03.015",
url = "http://www.sciencedirect.com/science/article/pii/S0377025706000826",
author = "Zhaosheng Yu and Anthony Wachs and Yannick Peysson",
}

@article{prashant2011,
title = "Direct simulations of spherical particle motion in {B}ingham liquids",
journal = "Computers \& Chemical Engineering",
volume = "35",
number = "7",
pages = "1200 - 1214",
year = "2011",
issn = "0098-1354",
doi = "https://doi.org/10.1016/j.compchemeng.2010.09.002",
url = "http://www.sciencedirect.com/science/article/pii/S0098135410003066",
author = " Prashant and J.J. Derksen",
}

@Article{fraggedakis2016,
author ="Fraggedakis, D. and Dimakopoulos, Y. and Tsamopoulos, J.",
title  ="Yielding the yield-stress analysis: a study focused on the effects of elasticity on the settling of a single spherical particle in simple yield-stress fluids",
journal  ="Soft Matter",
year  ="2016",
volume  ="12",
issue  ="24",
pages  ="5378-5401",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C6SM00480F",
url  ="http://dx.doi.org/10.1039/C6SM00480F",
}

@article{chaparian2018,
author = {Chaparian,Emad  and Wachs,Anthony  and Frigaard,Ian A. },
title = {Inline motion and hydrodynamic interaction of {2D} particles in a viscoplastic fluid},
journal = {Physics of Fluids},
volume = {30},
number = {3},
pages = {033101},
year = {2018},
doi = {10.1063/1.5022109},
URL = {https://doi.org/10.1063/1.5022109},
eprint = {https://doi.org/10.1063/1.5022109}
}

@article{singh2000,
title = "A distributed {L}agrange multiplier/fictitious domain method for viscoelastic particulate flows",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "91",
number = "2",
pages = "165 - 188",
year = "2000",
issn = "0377-0257",
doi = "https://doi.org/10.1016/S0377-0257(99)00104-4",
url = "http://www.sciencedirect.com/science/article/pii/S0377025799001044",
author = "P. Singh and D.D. Joseph and T.I. Hesla and R. Glowinski and T.-W. Pan",
}

@article{chaparian2018,
author = {Chaparian,Emad  and Wachs,Anthony  and Frigaard,Ian A. },
title = {Inline motion and hydrodynamic interaction of {2D} particles in a viscoplastic fluid},
journal = {Physics of Fluids},
volume = {30},
number = {3},
pages = {033101},
year = {2018},
doi = {10.1063/1.5022109},
URL = {https://doi.org/10.1063/1.5022109},
eprint = {https://doi.org/10.1063/1.5022109}
}

@article{koblitz2018,
  title = {Direct numerical simulation of particle sedimentation in a {B}ingham fluid},
  author = {Koblitz, A. R. and Lovett, S. and Nikiforakis, N.},
  journal = {Phys. Rev. Fluids},
  volume = {3},
  issue = {9},
  pages = {093302},
  numpages = {13},
  year = {2018},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevFluids.3.093302},
  url = {https://link.aps.org/doi/10.1103/PhysRevFluids.3.093302}
}

@Article{mitsoulis2017,
author="Mitsoulis, Evan and Tsamopoulos, John",
title="Numerical simulations of complex yield-stress fluid flows",
journal="Rheologica Acta",
year="2017",
month="Mar",
day="01",
volume="56",
number="3",
pages="231--258",
issn="1435-1528",
doi="10.1007/s00397-016-0981-0",
url="https://doi.org/10.1007/s00397-016-0981-0"
}

@Article{saramito2017,
author="Saramito, Pierre and Wachs, Anthony",
title="Progress in numerical simulation of yield stress fluid flows",
journal="Rheologica Acta",
year="2017",
month="Mar",
day="01",
volume="56",
number="3",
pages="211--230",
issn="1435-1528",
doi="10.1007/s00397-016-0985-9",
url="https://doi.org/10.1007/s00397-016-0985-9"
}

@article{tanner2019,
author = {Tanner,Roger I. },
title = {Review: {R}heology of noncolloidal suspensions with non-{N}ewtonian matrices},
journal = {Journal of Rheology},
volume = {63},
number = {4},
pages = {705-717},
year = {2019},
doi = {10.1122/1.5085363},
URL = {https://doi.org/10.1122/1.5085363},
eprint = {https://doi.org/10.1122/1.5085363}
}

@article{friggard2019,
title = "Simple yield stress fluids",
journal = "Current {O}pinion in {C}olloid \& Interface Science",
volume = "43",
pages = "80 - 93",
year = "2019",
issn = "1359-0294",
doi = "https://doi.org/10.1016/j.cocis.2019.03.002",
url = "http://www.sciencedirect.com/science/article/pii/S1359029419300068",
author = "Ian Frigaard",
}

@article{papanastasiou1987,
author = {Papanastasiou,Tasos C. },
title = {Flows of Materials with Yield},
journal = {Journal of Rheology},
volume = {31},
number = {5},
pages = {385-404},
year = {1987},
doi = {10.1122/1.549926},
URL = {https://doi.org/10.1122/1.549926},
eprint = {https://doi.org/10.1122/1.549926}
}

@book{glowinski1984,
  title={Numerical methods for nonlinear variational problems},
  author={Glowinski, R.},
  isbn={978-3-662-12613-4},
  url={https://doi.org/10.1007/978-3-662-12613-4},
  year={1984},
  publisher={Springer, Berlin, Heidelberg}
}

@InProceedings{tanner1983,
author =   {Tanner, R. I. and Milthorpe, J. F.},
title = {Numerical simulation of the flow of fluids with yield stress},
booktitle = {Num Meth Lam Turb Flow (Eds Taylor C, Johnson JA, Smith WR)},
  pages = {680-690},
  series = {Proc 3rd Int Conf (Seattle)},
  publisher = {Pineridge Press},
  address = {Swansea},
  year = {1983}
}

@article{beverly1989,
author = {Beverly,C. R.  and Tanner,R. I. },
title = {Numerical Analysis of Extrudate Swell in Viscoelastic Materials with Yield Stress},
journal = {Journal of Rheology},
volume = {33},
number = {6},
pages = {989-1009},
year = {1989},
doi = {10.1122/1.550042},
URL = {https://doi.org/10.1122/1.550042},
eprint = {https://doi.org/10.1122/1.550042}
}

@article{irving1950,
author = {Irving,J. H.  and Kirkwood,John G. },
title = {The Statistical Mechanical Theory of Transport Processes. {IV. T}he Equations of Hydrodynamics},
journal = {The Journal of Chemical Physics},
volume = {18},
number = {6},
pages = {817-829},
year = {1950},
doi = {10.1063/1.1747782},
URL = { https://doi.org/10.1063/1.1747782},
eprint = {https://doi.org/10.1063/1.1747782}
}

@article{adolfo2018_1,
  title = {Apparent slip mechanism between two spheres based on solvent rheology: {T}heory and implication for the shear thinning of non-{B}rownian suspensions},
  author = {V{\'a}zquez-Quesada, A. and Espa{\~n}ol, Pep and Ellero, M.},
  journal = {Phys. Rev. Fluids},
  volume = {3},
  issue = {12},
  pages = {123302},
  numpages = {14},
  year = {2018},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevFluids.3.123302},
  url = {https://link.aps.org/doi/10.1103/PhysRevFluids.3.123302}
}

@Article{kroupa2017,
author ="Kroupa, Martin and Soos, Miroslav and Kosek, Juraj",
title  ="Slip on a particle surface as the possible origin of shear thinning in non-{B}rownian suspensions",
journal  ="Phys. Chem. Chem. Phys.",
year  ="2017",
volume  ="19",
issue  ="8",
pages  ="5979-5984",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C6CP07666A",
url  ="http://dx.doi.org/10.1039/C6CP07666A",
}

@article{ness2015,
  title = {Flow regime transitions in dense non-{B}rownian suspensions: {R}heology, microstructural characterization, and constitutive modeling},
  author = {Ness, Christopher and Sun, Jin},
  journal = {Phys. Rev. E},
  volume = {91},
  issue = {1},
  pages = {012201},
  numpages = {10},
  year = {2015},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.91.012201},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.91.012201}
}

@article{bird2016,
  title = {The Rheology and Flow of Viscoplastic Materials},
  author = {Bird, R. B. and Dai, G. C. and  Yarusso, B. J. },
  journal = {Reviews in Chemical Engineering},
  volume = {1},
  issue = {1},
  pages = {1--70},
  year = {2016},
  publisher = {De Gruyter},
  doi = {10.1515/revce-1983-0102},
}

@article{kumar2010,
  title = {Origins of the anomalous stress behavior in charged colloidal suspensions under shear},
  author = {Kumar, Amit and Higdon, Jonathan J. L.},
  journal = {Phys. Rev. E},
  volume = {82},
  issue = {5},
  pages = {051401},
  numpages = {7},
  year = {2010},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.82.051401},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.82.051401}
}

@article{bolintineanu2014,
author="Bolintineanu, Dan S. and Grest, Gary S. and Lechman, Jeremy B. and Pierce, Flint and Plimpton, Steven J. and Schunk, P. Randall",
title="Particle dynamics modeling methods for colloid suspensions",
journal="Computational Particle Mechanics",
year="2014",
month="Sep",
day="01",
volume="1",
number="3",
pages="321--356",
issn="2196-4386",
doi="10.1007/s40571-014-0007-6",
url="https://doi.org/10.1007/s40571-014-0007-6"
}

@article{townsend2018,
author = {Townsend, Adam K.  and Wilson, Helen J. },
title = {Anomalous effect of turning off long-range mobility interactions in {S}tokesian dynamics},
journal = {Physics of Fluids},
volume = {30},
number = {7},
pages = {077103},
year = {2018},
doi = {10.1063/1.5031860},
URL = {https://doi.org/10.1063/1.5031860},
eprint = {https://doi.org/10.1063/1.5031860}
}

@article{adolfo2016_4,
  title = {Shear Thinning of Noncolloidal Suspensions},
  author = {V{\'a}zquez-Quesada, Adolfo and Tanner, Roger I. and Ellero, Marco},
  journal = {Phys. Rev. Lett.},
  volume = {117},
  issue = {10},
  pages = {108001},
  numpages = {5},
  year = {2016},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.117.108001},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.117.108001}
}

@article{hormozi2018, 
title={Interface-resolved simulations of particle suspensions in {N}ewtonian, shear thinning and shear thickening carrier fluids},
volume={852},
DOI={10.1017/jfm.2018.532},
journal={Journal of Fluid Mechanics},
publisher={Cambridge University Press},
author={Alghalibi, Dhiya and Lashgari, Iman and Brandt, Luca and Hormozi, Sarah},
year={2018},
pages={329–357}
}

@article{yang2018,
author = {Yang,Mengfei  and Shaqfeh,Eric S. G. },
title = {Mechanism of shear thickening in suspensions of rigid spheres in {B}oger fluids. {P}art {II: S}uspensions at finite concentration},
journal = {Journal of Rheology},
volume = {62},
number = {6},
pages = {1379-1396},
year = {2018},
doi = {10.1122/1.5024698},
URL = {https://doi.org/10.1122/1.5024698},
eprint = {https://doi.org/10.1122/1.5024698}
}

@article{liard2014,
author = {Liard,Maxime  and Martys,Nicos S.  and George,William L.  and Lootens, Didier  and Hebraud, Pascal },
title = {Scaling laws for the flow of generalized {N}ewtonian suspensions},
journal = {Journal of Rheology},
volume = {58},
number = {6},
pages = {1993-2015},
year = {2014},
doi = {10.1122/1.4896896},
URL = {https://doi.org/10.1122/1.4896896},
eprint = {https://doi.org/10.1122/1.4896896}
}

@article{adolfo2017_1,
title = "Investigating the causes of shear-thinning in non-colloidal suspensions: {E}xperiments and simulations",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "248",
pages = "1-7",
year = "2017",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2017.08.005",
url = "http://www.sciencedirect.com/science/article/pii/S0377025717301179",
author = "V{\'a}zquez-Quesada, Adolfo and Mahmud, Arif and Dai, Shaocong and Ellero, Marco and Tanner, Roger I.",
}

@article{hwang2004,
title = "Direct simulations of particle suspensions in a viscoelastic fluid in sliding bi-periodic frames",
journal = "Journal of Non-Newtonian Fluid Mechanics",
volume = "121",
number = "1",
pages = "15 - 33",
year = "2004",
issn = "0377-0257",
doi = "https://doi.org/10.1016/j.jnnfm.2004.03.008",
url = "http://www.sciencedirect.com/science/article/pii/S0377025704000655",
author = "Hwang, Wook Ryol and Hulsen, Martien A. and  Meijer, Han E.H.",
}

@Article{martys2010,
author="Martys, Nicos S. and George, William L. and Chun, Byong-Wa and Lootens, Didier",
title="A smoothed particle hydrodynamics-based fluid model with a spatially dependent viscosity: application to flow of a suspension with a non-{N}ewtonian fluid matrix",
journal="Rheologica Acta",
year="2010",
month="Oct",
day="01",
volume="49",
number="10",
pages="1059--1069",
issn="1435-1528",
doi="10.1007/s00397-010-0480-7",
url="https://doi.org/10.1007/s00397-010-0480-7"
}

@article{krishnan2017,
title = "Fully resolved viscoelastic particulate simulations using unstructured grids",
journal = "Journal of Computational Physics",
volume = "338",
pages = "313 - 338",
year = "2017",
issn = "0021-9991",
doi = "https://doi.org/10.1016/j.jcp.2017.02.068",
url = "http://www.sciencedirect.com/science/article/pii/S0021999117301717",
author = "Krishnan, Sreenath  and Shaqfeh, Eric S.G. and Iaccarino, Gianluca",
}

@article{koblitz2017,
title = "Direct numerical simulation of particulate flows with an overset grid method",
journal = "Journal of Computational Physics",
volume = "343",
pages = "414 - 431",
year = "2017",
issn = "0021-9991",
doi = "https://doi.org/10.1016/j.jcp.2017.04.058",
url = "http://www.sciencedirect.com/science/article/pii/S0021999117303376",
author = "Koblitz, A. R.  and Lovett, S.  and Nikiforakis, N.  and Henshaw, W.D. ",
}
@article{wachs2015,
title = "Accuracy of Finite Volume/Staggered Grid Distributed {L}agrange Multiplier/Fictitious Domain simulations of particulate flows",
journal = "Computers \& Fluids",
volume = "115",
pages = "154 - 172",
year = "2015",
issn = "0045-7930",
doi = "https://doi.org/10.1016/j.compfluid.2015.04.006",
url = "http://www.sciencedirect.com/science/article/pii/S0045793015001152",
author = " Wachs, Anthony and Hammouti, Abdelkader  and  Vinay, Guillaume and Rahmani, Mona ",
}
@article{fiore2019, 
title={Fast {S}tokesian dynamics}, 
volume={878}, 
DOI={10.1017/jfm.2019.640}, 
journal={Journal of Fluid Mechanics}, 
publisher={Cambridge University Press}, 
author={Fiore, Andrew M. and Swan, James W.}, 
year={2019}, 
pages={544–597}
}
@article{gallier2018,
  title = {Simulations of sheared dense noncolloidal suspensions: {E}valuation of the role of long-range hydrodynamics},
  author = {Gallier, Stany and Peters, Fran\c{c}ois and Lobry, Laurent},
  journal = {Phys. Rev. Fluids},
  volume = {3},
  issue = {4},
  pages = {042301},
  numpages = {9},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevFluids.3.042301},
  url = {https://link.aps.org/doi/10.1103/PhysRevFluids.3.042301}
}
@book{kim2005,
  title={Microhydrodynamics: {P}rinciples and Selected Applications},
  author={Kim, S. and Karrila, S.J.},
  isbn={9780486442198},
  lccn={2005041157},
  series={Butterworth - Heinemann series in chemical engineering},
  year={2005},
  publisher={Dover Publications}
}
@article{adolfo2018_2,
author = {V{\'a}zquez-Quesada, A.  and Wagner, N. J.  and Ellero, M. },
title = {Normal lubrication force between spherical particles immersed in a shear-thickening fluid},
journal = {Physics of Fluids},
volume = {30},
number = {12},
pages = {123102},
year = {2018},
doi = {10.1063/1.5054067},
URL = {https://doi.org/10.1063/1.5054067},
eprint = {https://doi.org/10.1063/1.5054067}
}
@article{gurnon2015, 
title={Microstructure and rheology relationships for shear thickening colloidal dispersions}, 
volume={769}, 
DOI={10.1017/jfm.2015.128}, 
journal={Journal of Fluid Mechanics}, 
publisher={Cambridge University Press}, 
author={Gurnon, A. Kate and Wagner, Norman J.}, 
year={2015}, 
pages={242–276}
}
@article{bian2014,
title = "A splitting integration scheme for the {SPH} simulation of concentrated particle suspensions",
journal = "Computer Physics Communications",
volume = "185",
number = "1",
pages = "53 - 62",
year = "2014",
issn = "0010-4655",
doi = "https://doi.org/10.1016/j.cpc.2013.08.015",
url = "http://www.sciencedirect.com/science/article/pii/S0010465513002786",
author = "Bian, Xin and Ellero, Marco",
}
@article{banchio2003,
author = {Banchio,Adolfo J.  and Brady,John F. },
title = {Accelerated {S}tokesian dynamics: {B}rownian motion},
journal = {The Journal of Chemical Physics},
volume = {118},
number = {22},
pages = {10323-10332},
year = {2003},
doi = {10.1063/1.1571819},
URL = {https://doi.org/10.1063/1.1571819},
eprint = {https://doi.org/10.1063/1.1571819}
}
@article{adolfo2019_1, 
title={Shear thickening of a non-colloidal suspension with a viscoelastic matrix}, volume={880}, 
DOI={10.1017/jfm.2019.753}, 
journal={Journal of Fluid Mechanics}, 
publisher={Cambridge University Press}, 
author={V\'{a}zquez-Quesada, Adolfo and Espa\~{n}ol, Pep and Tanner, Roger I. and Ellero, Marco}, 
year={2019}, 
pages={1070–1094}
}
@article{cox1967,
title = "The slow motion of a sphere through a viscous fluid towards a plane surface-{II} {S}mall gap widths, including inertial effects",
journal = "Chemical Engineering Science",
volume = "22",
number = "12",
pages = "1753 - 1777",
year = "1967",
issn = "0009-2509",
doi = "https://doi.org/10.1016/0009-2509(67)80208-2",
url = "http://www.sciencedirect.com/science/article/pii/0009250967802082",
author = "Cox, R. G. and Brenner, H.",
}
@article{goldman1967,
title = "Slow viscous motion of a sphere parallel to a plane wall-{I.} {M}otion through a quiescent fluid",
journal = "Chemical Engineering Science",
volume = "22",
number = "4",
pages = "637 - 651",
year = "1967",
issn = "0009-2509",
doi = "https://doi.org/10.1016/0009-2509(67)80047-2",
url = "http://www.sciencedirect.com/science/article/pii/0009250967800472",
author = "Goldman, A. J. and Cox, R. G. and Brenner, H.",
}

@article{jeffery1982,
author = {Jeffrey, D. J.},
title = {Low-{R}eynolds-number flow between converging spheres},
journal = {Mathematika},
volume = {29},
number = {1},
pages = {58-66},
doi = {10.1112/S002557930001216X},
url = {https://londmathsoc.onlinelibrary.wiley.com/doi/abs/10.1112/S002557930001216X},
year = {1982}
}

@ARTICLE{PThien1994,
author={Phan-Thien, N. and Kim, S.},
title={The load transfer between two rigid spherical inclusions in an elastic medium},
journal={{ZAMP} {Z}eitschrift f{\"u}r angewandte {M}athematik und {P}hysik},
year={1994},
volume={45},
number={2},
pages={177-201},
doi={10.1007/BF00943501},
url = {https://doi.org/10.1007/BF00943501}
}

@article{groot1997,
author = {Groot,Robert D.  and Warren,Patrick B. },
title = {Dissipative particle dynamics: {B}ridging the gap between atomistic and mesoscopic simulation},
journal = {The Journal of Chemical Physics},
volume = {107},
number = {11},
pages = {4423-4435},
year = {1997},
doi = {10.1063/1.474784},
URL = {https://doi.org/10.1063/1.474784}
}



